Query-by-Example Keyword Spotting system using Multi-head Attention and Softtriple Loss

This paper proposes a neural network architecture for tackling the query-by-example user-defined keyword spotting task. A multi-head attention module is added on top of a multi-layered GRU for effective feature extraction, and a normalized multi-head attention module is proposed for feature aggregation. We also adopt the softtriple loss - a combination of triplet loss and softmax loss - and showcase its effectiveness. We demonstrate the performance of our model on internal datasets with different languages and the public Hey-Snips dataset. We compare the performance of our model to a baseline system and conduct an ablation study to show the benefit of each component in our architecture. The proposed work shows solid performance while preserving simplicity.

==> archive/rebuttal.tex <==
Reviewer 1

We thank reviewer 1774 for their review and suggestion. The concern about about lacking comparison with other approaches on different corpora has been addressed below:

Keyword spotting have been studied many times, but, there are only a few user defined key word spotting papers available, among which the methods proposed by Chen et al. [1] is the one most close to our problem, which uses text-independent QbyE system. 
During our development, we used [1] as baseline. Our model shows a huge performance gain compare to [1]. We add experiments to our best configed model from [1] to both our internal data and the Hey-Snips dataset, the results are showing below:
Results 1:




We also compared our methods with the tanh attention mechanism from Chowdhury et al. [2], the tanh attention mechanism is a one of the state-of-the-art algorithm which was developed for speaker verification task, it has been implemented in multiple papers in speaker verification and keyword spotting [3][4]. Our comparison to [2] (in Section 4.3) is: [2] adds more parameters while achieving comparable performance with our Non-normalized multi-head attention aggregator. In comparing [2] with our Normalized multi-head attention aggreagor (normalization is one of our major contribution to this paper), our normalized multi-head attention mechanism shows significant FRR deduction (from 7.22% to 5.28% on our small model, from 7.99% to 3.99% on our large model).


In order to further compare our methods to the more classical methods, we add another experiment to combine [1] and [2], in which we used the RNN encoder and softmax loss from [1], and the attention mechanism from [2]. Compare the results 2 to the above results 1 shows that, in general, adding attention performs better than pure RNN-based results from [1]. Compare results 2 to our model performance reported in the paper, we conclude that our attention components has better performance than [2].
Results 2:




The reviewer also pointed out that we should compare our methods on different corpora:


Literatures in user-defined kws often use internal dataset to test their algorithms, we used both internal and public available Hey-Snips dataset to illustrate the algorithm performances under clean and babble senarios with different model parameter settings. We are the first to use the public available dataset to show the performane. We also detailed our evaluation methods on the Hey-Snips dataset, hope it can be build as a baseline for future research.


Hey-Snapdragon is another public available dataset which can be used for user-defined keyword spotting task, however, unlike Hey-Snips, Hey-Snapdragon doesn't provide negative samples, which makes the evaluation ...


More experiments on baseline algorithms with the internal and Hey-Snips dataset are performed, results are showing above, and can be reported in the next version of our paper. 


[1] Chen, Guoguo, Carolina Parada, and Tara N. Sainath. "Query-by-example keyword spotting using long short-term memory networks." 2015 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP). IEEE, 2015.


[2] rahman Chowdhury, FA Rezaur, et al. "Attention-based models for text-dependent speaker verification." 2018 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP). IEEE, 2018.


[3] Dey, Subhadeep, Srikanth R. Madikeri, and Petr Motlicek. "End-to-end Text-dependent Speaker Verification Using Novel Distance Measures." INTERSPEECH. 2018.


[4] Lee, Mingu, et al. "Orthogonality Constrained Multi-Head Attention for Keyword Spotting." 2019 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU). IEEE, 2019.

Reviewer 3

We thank reviewer 2520 for their review and providing feedback for section 4.3 as well as table 1. We added the definitions of the abbreviations in table 1's description. Regarding the results in 4.3, we added more details and made the comparisons more explicit. Thank you for pointing this out.
